Cream Skimming the Underground: Identifying Relevant Information Points from Online Forums

This paper proposes a machine learning-based approach for detecting the exploitation of vulnerabilities in the wild by monitoring underground hacking forums. The increasing volume of posts discussing exploitation in the wild calls for an automatic approach to process threads and posts that will eventually trigger alarms depending on their content. To illustrate the proposed system, we use the CrimeBB dataset, which contains data scraped from multiple underground forums, and develop a supervised machine learning model that can filter threads citing CVEs and label them as Proof-of-Concept, Weaponization, or Exploitation. Leveraging random forests, we indicate that accuracy, precision and recall above 0.99 are attainable for the classification task. Additionally, we provide insights into the difference in nature between weaponization and exploitation, e.g., interpreting the output of a decision tree, and analyze the profits and other aspects related to the hacking communities. Overall, our work sheds insight into the exploitation of vulnerabilities in the wild and can be used to provide additional ground truth to models such as EPSS and Expected Exploitability.

==> futurework.tex <==
https://docs.google.com/document/d/1jxv6cSzCrfDqsRbuHDsPi7aQTby9edW_zxXsX9MimpQ/edit?usp=sharing






 

Cainã: draw trees



Felipe: 

* performance of algorithms, in tree


* table with other algorithms, beyond decision tree


* árvore de decisão que dividem entre Exploitation vs Rest (PoC  + Weaponization) -- consider many more possibilities, including decision trees to filter single tags (PoC or non-PoC; tutorial or non-tutorial; etc)



Felipe:

Felipe já fez, falta passar para artigo:  criar história junto com Cainã. 

10 boxplots -- 5 CVSS e 5 EPSS, não ponderados  (PoC, Weaponization, Exploitatioon, All in our dataset, All over NVD)

8 boxplots -- 4 CVSS e 4 EPSS,  ponderados (PoC, Weaponization, Exploitatioon, All in our dataset)

EPSS ao longo do tempo, 5 linhas, não ponderadas

EPSS ao longo do tempo, 4 linhas,  ponderadas




========================================================================


depois de segunda-feira



\textcolor{red}{FUTURE WORK: filter from CrimeBB CVES ONLY from exploitation threads}


\textcolor{red}{Present statistics about CVEs for which we found information about exploitation at CrimeBB, but for which we did not find any exploits neither at Github nor at ExploitDB}

 % The detector has an accuracy of  x\% and an  f1-score of y\%.  


 
 
* named vulnerabilities


* usar ChatGPT para classificar posts (semelhante ao que foi feito no artigo do GitHub)
